Construction and Hedging of Equity Index Options Portfolios

This research presents a comprehensive evaluation of systematic index option-writing strategies, focusing on S&P500 index options. We compare the performance of hedging strategies using the Black-Scholes-Merton (BSM) model and the Variance-Gamma (VG) model, emphasizing varying moneyness levels and different sizing methods based on delta and the VIX Index. The study employs 1-minute data of S&P500 index options and index quotes spanning from 2018 to 2023. The analysis benchmarks hedged strategies against buy-and-hold and naked option-writing strategies, with a focus on risk-adjusted performance metrics including transaction costs. Portfolio delta approximations are derived using implied volatility for the BSM model and market-calibrated parameters for the VG model. Key findings reveal that systematic option-writing strategies can potentially yield superior returns compared to buy-and-hold benchmarks. The BSM model generally provided better hedging outcomes than the VG model, although the VG model showed profitability in certain naked strategies as a tool for position sizing. In terms of rehedging frequency, we found that intraday hedging in 130-minute intervals provided both reliable protection against adverse market movements and a satisfactory returns profile.

==> metrics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[!ht]
\centering
\caption{Performance metrics definitions.}
\label{tab:performance-metrics}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccc@{}}
\toprule
Metric &
  Abbreviation &
  Formula &
  Additional Information \\ \midrule \addlinespace[0.75em]
Daily Returns &
  r &
  $r_i:=\frac{p_i - p_{i-1}}{p_t}$ &
  $p_t$ is asset price on day $i$ of backtest \\ \addlinespace[0.75em]
Annualized Compounded Returns &
  aRC &
  $ARC:=\prod_{i=1}^{n}(1+r_i^{\frac{252}{n}}) - 1$ &
  $n$ is the number of days in the whole backtesting period \\ \addlinespace[0.75em]
Annualized Standard Deviation &
  aSD &
  $aSD:=\sqrt{252} \cdot \sqrt{\frac{1}{n-1}\sum_{i=1}^{n}(r_i - \overline{r})^2}$ &
  $\overline{r}$ is the average of daily returns \\ \addlinespace[0.75em]
Maximum Drawdown &
  MD &
  $MD:=\sup_{(x, y)\in\big\{(t_i, t_j) \in \mathbb{R}: t_i < t_j\big\}}\frac{p_x - p_y}{p_x}$ &
  $p$ is the total equity value \\ \addlinespace[0.75em]
Maximum Loss Duration &
  MLD &
  $MLD:=\frac{y-x}{252}$ &
  \begin{tabular}[c]{@{}c@{}}$x, y$ are days defined in formula MD formula and indicate\\  days of consecutive local maxima of the equity values\end{tabular} \\
Information Ratio &
  IR &
  $IR:=\frac{aRC}{aSD}$ &
   \\ \addlinespace[0.75em]
Information Ratio ** &
  IR** &
  $IR^{**}:=\frac{IR \cdot sign(aRC) \cdot aRC}{MD}$ &
   \\ \addlinespace[0.75em]
Information Ratio *** &
  IR*** &
  $IR^{***}:=\frac{aRC^3}{aSD \cdot MD \cdot MLD} * 1000$ &
   \\ \addlinespace[0.75em]
Value-at-Risk &
  VaR &
  $VaR_{\alpha}(X) := -\inf\big\{x \in \mathbb{R}: F_{X}(x) \geq \alpha \big\}$ &
  Historical VaR of portfolio returns at a 95\% confidence level \\ \addlinespace[0.75em]
Conditional Value-at-Risk &
  CVaR &
  $CVaR_{\alpha}{X}:=-\frac{1}{\alpha}\int_{0}^{\alpha} VaR(\gamma)d\gamma$ &
  \begin{tabular}[c]{@{}c@{}}CVaR (expected shortfall, ES) estimated as the \\ average of returns below $VaR_{\alpha}(X)$\end{tabular} \\  \bottomrule
\end{tabular}%
}
\source{Each year is assumed to have 252 trading days.}
\end{table}
